On the Throughput/Bit-Cost Tradeoff in CSMA Based Cooperative Networks

Wireless local area networks (WLAN) still suffer from a severe performance discrepancy between different users in the uplink. This is because of the spatially varying channel conditions provided by the wireless medium. Cooperative medium access control (MAC) protocols as for example CoopMAC were proposed to mitigate this problem. In this work, it is shown that cooperation implies for cooperating nodes a tradeoff between throughput and bit-cost, which is the energy needed to transmit one bit. The tradeoff depends on the degree of cooperation. For carrier sense multiple access (CSMA) based networks, the throughput/bit-cost tradeoff curve is theoretically derived. A new distributed CSMA protocol called fairMAC is proposed and it is theoretically shown that fairMAC can asymptotically achieve any operating point on the tradeoff curve when the packet lengths go to infinity. The theoretical results are validated through Monte Carlo simulations.

==> Makefile <==
PROJECT=fairMAC
TMPFILES=*.aux *.bak *.bbl *.blg *.lof *.log *.toc *.lot *~ *.backup\
*.pfx *.ovp $(PROJECT)-pics.* $(PROJECT).dvi $(PROJECT).ps

default: 
	latex $(PROJECT).tex;
	dvips -o $(PROJECT).ps $(PROJECT).dvi;
	ps2pdf14 -sPAPERSIZE=letter -dPDFSETTINGS=/prepress $(PROJECT).ps;

clean:
	rm -f $(TMPFILES);
clean_pdf:
	rm -f $(PROJECT).pdf;

$(PROJECT).tex: clean_pdf
	latex $(PROJECT).tex;
	dvips -o $(PROJECT).ps $(PROJECT).dvi;
	ps2pdf14 -sPAPERSIZE=letter -dPDFSETTINGS=/prepress $(PROJECT).ps;

bib:	
	bibtex $(PROJECT);

literatur:
	cp ../references/Literatur.bib ./;
	cp ../references/confs-jrnls.bib ./;

final: clean clean_pdf
	latex $(PROJECT).tex;
	latex $(PROJECT).tex;
	bibtex $(PROJECT);
	latex $(PROJECT).tex;
	latex $(PROJECT).tex;
	dvips -o $(PROJECT).ps $(PROJECT).dvi;
	ps2pdf14 -sPAPERSIZE=letter -dPDFSETTINGS=/prepress $(PROJECT).ps;
	pdffonts $(PROJECT).pdf;

arxiv:
	rm -f $(PROJECT).aux $(PROJECT).blg $(PROJECT).dvi $(PROJECT).log $(PROJECT).pdf $(PROJECT).ps *.bib *~ .*.xml;



==> diagram.tex <==
\newcommand{\shortarrow}{\!\!\rightarrow\!\!}
\begin{figure*}
\centering
\subfloat[fairMAC with $P=1$, $Q=0$. The upper timeline displays one round of Direct Link. The lower timeline displays the transition phase of fairMAC and one round in steady state. This can be seen from investigating the state vector. Both at the beginning and at the end of a round in steady state it has to be of the same value, which is the case here. As can be seen, fairMAC with $P=1$, $Q=0$ in steady state is equivalent to Direct Link.]
{
\footnotesize
\psfrag{-1 s}{$-1$ s}
\psfrag{0 s}{0 s}
\psfrag{1 s}{1 s}
\psfrag{2 s}{2 s}
\psfrag{Direct Link}{Direct Link}
\psfrag{transition phase}{transition phase}
\psfrag{fairMAC}{fairMAC with $P=1$, $Q=0$ in steady state}
\psfrag{s1h}{\color{black}{$1\shortarrow 3$}}
\psfrag{s2h}{\color{black}{$2\shortarrow 3$}}
\psfrag{h1d}{\color{black}{$3\shortarrow\mathrm{ap}$}}
\psfrag{h2d}{\color{black}{$3\shortarrow\mathrm{ap}$}}
\psfrag{hd}{\color{black}{$3\shortarrow\mathrm{ap}$}}
\psfrag{s1d}{\color{black}{$1\shortarrow\mathrm{ap}$}}
\psfrag{s2d}{\color{black}{$2\shortarrow\mathrm{ap}$}}
\psfrag{data0}{
$\left[\!\!
\begin{array}{l}
0\\
0\\
\emptyset
\end{array}
\!\!\!
\right]
$
}
\psfrag{data1}{
$\left[\!\!
\begin{array}{l}
1\\
0\\
n_1
\end{array}
\!\!\!
\right]
$
}
\psfrag{data2}{
$\left[\!\!\!
\begin{array}{l}
1\\
1\\
n_1n_2
\end{array}
\!\!\!\!
\right]
$
}
\includegraphics[height=0.25\textwidth]{figures/RRqzero.eps}
\label{fig:RRqzero}
}
\hfill
\subfloat[fairMAC with $P=1$, $Q=2$. In the upper timeline, one round of CoopMAC is displayed. In the lower timeline, one round of fairMAC is shown. By reordering the packets, it can be seen that fairMAC with $P=1$, $Q=2$ is equivalent to CoopMAC in terms of throughput and bit-cost.]
{
\footnotesize
\psfrag{-1 s}{$-1$ s}
\psfrag{0 s}{0 s}
\psfrag{1 s}{1 s}
\psfrag{coopMAC}{CoopMAC}
\psfrag{transition phase}{transition phase}
\psfrag{fairMAC}{fairMAC with $P=1$, $Q=2$}
\psfrag{s1h}{\color{black}{$1\shortarrow 3$}}
\psfrag{s2h}{\color{black}{$2\shortarrow 3$}}
\psfrag{h1d}{\color{black}{$3\shortarrow\mathrm{ap}$}}
\psfrag{h2d}{\color{black}{$3\shortarrow\mathrm{ap}$}}
\psfrag{hd}{\color{black}{$3\shortarrow\mathrm{ap}$}}
\psfrag{s1d}{\color{black}{$1\shortarrow\mathrm{ap}$}}
\psfrag{s2d}{\color{black}{$2\shortarrow\mathrm{ap}$}}
\psfrag{data0}{
$\left[\!\!
\begin{array}{l}
0\\
0\\
\emptyset
\end{array}
\!\!\!
\right]
$
}
\psfrag{data1}{
$\left[\!\!
\begin{array}{l}
1\\
0\\
n_1
\end{array}
\!\!\!
\right]
$
}
\psfrag{data2}{
$\left[\!\!
\begin{array}{l}
1\\
1\\
n_1n_2
\end{array}
\!\!\!
\right]
$
}
\psfrag{data3}{
$\left[\!\!
\begin{array}{l}
0\\
0\\
\emptyset
\end{array}
\!\!\!
\right]
$
}
\includegraphics[height=0.25\textwidth]{figures/RRqtwo.eps}
\label{fig:RRqtwo}
}
\\
\subfloat[fairMAC with $P=Q=1$. In the upper timeline, one round of time sharing between CoopMAC and Direct Link with $\alpha=5/12$ is displayed. One such round consists of one round of Direct Link followed by one round of CoopMAC. In the lower timeline, the transition phase of fairMAC and one round in steady state are displayed. Note that the fairMAC state vector at the beginning of the steady state round equals the state vector at the end of the steady state round. By reordering the packets, we see that fairMAC with $P=1$ and $Q=2$ reaches the operating point of timesharing between CoopMAC and Direct Link at $\alpha=5/12$.]
{
\footnotesize
\psfrag{-1 s}{$-1$ s}
\psfrag{0 s}{0 s}
\psfrag{1 s}{1 s}
\psfrag{2 s}{2 s}
\psfrag{3 s}{3 s}
\psfrag{4 s}{4 s}
\psfrag{Direct Link}{Direct Link}
\psfrag{coopMAC}{CoopMAC}
\psfrag{transition phase}{transition phase}
\psfrag{fairMAC}{fairMAC with $P=Q=1$ in steady state}
\psfrag{s1h}{\color{black}{$1\shortarrow 3$}}
\psfrag{s2h}{\color{black}{$2\shortarrow 3$}}
\psfrag{h1d}{\color{black}{$3\shortarrow\mathrm{ap}$}}
\psfrag{h2d}{\color{black}{$3\shortarrow\mathrm{ap}$}}
\psfrag{hd}{\color{black}{$3\shortarrow\mathrm{ap}$}}
\psfrag{s1d}{\color{black}{$1\shortarrow\mathrm{ap}$}}
\psfrag{s2d}{\color{black}{$2\shortarrow\mathrm{ap}$}}
\psfrag{data0}{
$\left[\!\!
\begin{array}{l}
0\\
0\\
\emptyset
\end{array}
\!\!\!
\right]
$
}
\psfrag{data1}{
$\left[\!\!
\begin{array}{l}
1\\
0\\
n_1
\end{array}
\!\!\!
\right]
$
}
\psfrag{data2}{
$\left[\!\!
\begin{array}{l}
1\\
1\\
n_1n_2
\end{array}
\!\!\!
\right]
$
}
\psfrag{data3}{
$\left[\!\!
\begin{array}{l}
0\\
1\\
n_2
\end{array}
\!\!\!
\right]
$
}
\psfrag{data4}{
$\left[\!\!
\begin{array}{l}
1\\
1\\
n_2n_1
\end{array}
\!\!\!
\right]
$
}
\psfrag{data5}{
$\left[\!\!
\begin{array}{l}
1\\
0\\
n_1
\end{array}
\!\!\!
\right]
$
}
\psfrag{data6}{
$\left[\!\!
\begin{array}{l}
1\\
1\\
n_1n_2
\end{array}
\!\!\!
\right]
$
}
\psfrag{data7}{
$\left[\!\!
\begin{array}{l}
0\\
1\\
n_2
\end{array}
\!\!\!
\right]
$
}
\includegraphics[height=0.25\textwidth]{figures/RRqone.eps}
\label{fig:RRqone}
}
\caption{A diagram that visualizes the behavior of Round Robin based Direct Link, CoopMAC and fairMAC. Transmissions of $n_k$ to the AP are denoted by $k\rightarrow \mathrm{ap}$, $k=1,2,3$. Transmissions to the helper $n_3$ are denoted by $k\rightarrow 3$, $k=1,2$. To facilitate orientation in the diagrams, transmissions of $n_1$ are marked red, transmissions of $n_2$ are marked green, and transmissions of $n_3$ are left white. When $n_3$ forwards data of $n_1$, the corresponding packet is marked by a red bar, and when $n_3$ forwards data of $n_2$, the corresponding packet is marked by a green bar. For fairMAC, the network state can be described by the number $p_1$ of pending packets at $n_1$, the number $p_2$ of pending packets at $n_2$ and the state of the forwarding queue $q$ at $n_3$. These state variables are displayed together in the vector $[p_1\,p_2\, q]$ transposed.}
 \label{fig:RRdiagram}
\end{figure*}

